MixUp as Directional Adversarial Training

In this work, we explain the working mechanism of MixUp in terms of adversarial training. We introduce a new class of adversarial training schemes, which we refer to as directional adversarial training, or DAT. In a nutshell, a DAT scheme perturbs a training example in the direction of another example but keeps its original label as the training target. We prove that MixUp is equivalent to a special subclass of DAT, in that it has the same expected loss function and corresponds to the same optimization problem asymptotically. This understanding not only serves to explain the effectiveness of MixUp, but also reveals a more general family of MixUp schemes, which we call Untied MixUp. We prove that the family of Untied MixUp schemes is equivalent to the entire class of DAT schemes. We establish empirically the existence of Untied Mixup schemes which improve upon MixUp.

==> supplement_main.tex <==



%%%% mixup converge result 1
%
%\begin{lem}
%\label{lem:mixUpConverge1}
%For any fixed infinite sequence $(x, x')_1^\infty$ and any infinite sequence of i.i.d. random variables $\Lambda_1^\infty$ drawn from $P^{\rm Mix}$, let 
%${\cal L}^{\rm Mix}\left((x, x' )_1^K, \Lambda_1^K \right)$ be defined according to (\ref{eq:Lmix}), with the first $K$ elements of $(x, x')_1^\infty$ and the first $K$ elements of $\Lambda_1^\infty$ as input. Let
%\[
%\delta_{\rm Mix}: = \max_{(x, x') \in {\cal D} \times {\cal D}}  \sup_{(\lambda, \lambda') \in [0, 1]\times [0, 1]} \left| \ell^{\rm Mix}(x, x', \lambda) - \ell^{\rm Mix}(x, x', \lambda') \right| .
%\]
%Then  for any $\epsilon >0$, 
%\[
%{\rm Pr}\left[
%\left|
%{\cal L}^{\rm Mix}\left(
%(x, x')_1^K, \Lambda_1^K
%\right) -  {\cal L}^{\rm Mix}\left(
%\left(x, x'\right)_1^K
%\right) 
%\right| \ge \epsilon
%\right]
%<
%2 \exp \left( -  \frac{2\epsilon^2}{\delta_{\rm Mix}^2} \cdot K\right).
%\]
%\end{lem}

\subsection*{Proof of Lemma 2:} 


For any given $\lambda_1^K\in [0, 1]^K$ and any of its modified version $u_1^K\in [0, 1]^K$ which differs from $\lambda_1^K$ in exactly one location, it can be verify, 
following the definition of $\delta_{\rm Mix}$, that
\[
\left|
{\cal L}^{\rm Mix}\left(
(x, x')_1^K, \lambda_1^K
\right) - 
{\cal L}^{\rm Mix}\left(
(x, x')_1^K, u_1^K
\right) 
\right| \le \delta_{\rm Mix}/K
\]
Since $\Lambda_1, \Lambda_2, \ldots \Lambda_K$ are independent and by McDiarmid Inequality \cite{mcdiarmid1989method}, it follows that  for any $\epsilon >0$, 
\[
{\rm Pr}\left[
\left|
{\cal L}^{\rm Mix}\left(
(x, x')_1^K, \Lambda_1^K
\right) -  {\cal L}^{\rm Mix}\left(
\left(x, x'\right)_1^K
\right) 
\right| \ge \epsilon
\right]
<
2 \exp \left( - \frac{2\epsilon^2}{K\cdot \left( \delta_{\rm Mix}/K\right)^2}\right) 
\]
which proves the lemma \hfill $\Box$



%%%%%%%%%%%%%%% DAT %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%





%%%%%%%%%%%%%%%%%%  MixUp vs DAT. %%%%%%%%%%%%%%%%%%%%




%\begin{thm}
%\label{thm:MixDATequalExp}
% Let $(x, x')_1^K$ be a sequence of object pairs on which MixUp with policy $P^{\rm Mix}$ and DAT with policy $P^{\rm DAT}$ will apply independently.  If $(x, x')_1^K$ is symmetric and $P^{\rm DAT} = {\mathbb D}(P^{\rm Mix})$, then
%\[
%{\cal L}^{\rm Mix}\left((x, x')_1^K \right) = {\cal L}^{\rm DAT}\left((x, x')_1^K \right) 
%\]
%\end{thm}

\subsection*{Proof of Theorem 1:}

\begin{eqnarray*}
{\cal L}^{\rm Mix} \left((x, x')_1^K \right) 
\!\!\!\!\!\!\!\!\!\!\!\!\!& = & 
\frac{1}{K}\sum\limits_{k=1}^K  {\mathbb E}_{\lambda_k \sim P^{\rm Mix}} \ell^{\rm Mix}(x_k,  x'_k, \lambda_k)\\
%&\stackrel{({\rm Lemma}~ \ref{lem:key})}{=} & 
%\frac{1}{K}\sum\limits_{k=1}^K  {\mathbb E}_{\Lambda_k} {\mathbb E}_{W_k|\Lambda_k} 
%\left\{
%W_k \ell^{\rm DAT}(x_k\rightarrow x'_k, \Lambda_k)
%+
%(1-W_k) \ell^{\rm DAT}(x'_k\rightarrow x_k, \overline{\Lambda_k})
%\right\} \\
&\stackrel{({\rm Lemma}~ \ref{lem:key})}{=} &
\frac{1}{K}
\left\{
\sum\limits_{k=1}^K \int \lambda P^{\rm Mix}(\lambda) \ell^{\rm DAT}(x_k\rightarrow x'_k, \lambda) d\lambda
+ 
\sum\limits_{k=1}^K \int \overline{\lambda} P^{\rm Mix}(\lambda) \ell^{\rm DAT}(x'_k\rightarrow x_k, \overline{\lambda}) d\lambda
\right\}\\
& \stackrel{({\rm symmetry})}= & 
\frac{1}{K}
\left\{
\sum\limits_{k=1}^K \int \lambda P^{\rm Mix}(\lambda) \ell^{\rm DAT}(x_k\rightarrow x'_k, \lambda) d\lambda
+ 
\sum\limits_{k=1}^K \int \overline{\lambda} P^{\rm Mix}(\lambda) \ell^{\rm DAT}(x_k\rightarrow x'_k, \overline{\lambda}) d\lambda
\right\}\\
& = & 
\frac{1}{K}
\left\{
\sum\limits_{k=1}^K \int \lambda P^{\rm Mix}(\lambda) \ell^{\rm DAT}(x_k\rightarrow x'_k, \lambda) d\lambda
+ 
\sum\limits_{k=1}^K \int \lambda P^{\rm Mix}(1-\lambda) \ell^{\rm DAT}(x_k\rightarrow x'_k, \lambda) d\lambda
\right\}\\
& = & 
\frac{1}{K}
\sum\limits_{k=1}^K 
\int \lambda \left(
P^{\rm Mix}(\lambda) +P^{\rm Mix}(1-\lambda)
\right)
\ell^{\rm DAT}(x_k\rightarrow x'_k, \lambda) d\lambda
\\
& = & 
\frac{1}{K}
\sum\limits_{k=1}^K 
\int P^{\rm DAT}(\lambda)
\ell^{\rm DAT}(x_k\rightarrow x'_k, \lambda) d\lambda
\\
& = & 
\frac{1}{K}
\sum\limits_{k=1}^K 
{\mathbb E}_{\lambda_k\sim P^{\rm DAT}} \ell^{\rm DAT}(x_k\rightarrow x'_k, \lambda_k)\\
& = & {\cal L}^{\rm DAT}\left( (x, x')_1^K\right)
\end{eqnarray*}
This completes the proof. \hfill $\Box$





%%%%%%%%%%%%%%%%%%%%%%%. untied mixup. %%%%%%%%%%%%%%%%%%





%%%% mixup converge result 1


%%%%%%%%%%%%%%%%%%%% untied MixUp Vs DAT %%%%%%%%%%%%%%%%%%%%%%%%%%






%\begin{thm}
%\label{thm:uMixDATequalExp}
% Let $(x, x')_1^K$ be a sequence of object pairs on which an Untied MixUp specified by $(P^{\rm Mix}, \gamma)$ and a DAT scheme with policy $P^{\rm DAT}$ will apply independently.  If $(x, x')_1^K$ is symmetric and $\left(P^{\rm Mix}, \gamma\right) = {\mathbb U}(P^{\rm DAT})$, then
%\[
%{\cal L}^{\rm uMix}\left((x, x')_1^K, \gamma\right) = {\cal L}^{\rm DAT}\left((x, x')_1^K \right) 
%\]
%\end{thm}


\subsection* {Proof of Theorem 3:} 
\begin{eqnarray*}
{\cal L}^{\rm uMix}
\left(
(x, x')_1^K, \gamma
\right)
& \!\!\!\!\!\! := & \!\!\!\!\!\!
 \frac{1}{K}
 \sum\limits_{k=1}^K 
 {\mathbb E}_{\lambda \sim P^{\rm Mix}} 
 \left\{
 \gamma(\lambda) \ell^{\rm DAT}(x_k \rightarrow x'_k, \lambda)
 + \overline{\gamma(\lambda)} \ell^{\rm DAT}(x'_k \rightarrow x_k, \overline{\lambda})
 \right\} \\
& = & \!\!\!\!\!\!
 \frac{1}{K}
 \sum\limits_{k=1}^K 
 \int
 \left(
 \gamma(\lambda) P^{\rm Mix}(\lambda)
  \ell^{\rm DAT}(x_k \rightarrow x'_k, \lambda) \right. 
\left.
 + 
\overline{ \gamma(\lambda)} P^{\rm Mix}(\lambda)
 \ell^{\rm DAT}(x'_k \rightarrow x_k,  \overline{\lambda})
 \right)
 d\lambda \\
 % & = & \!\!\!\!\!\!
% \frac{1}{K}
% \sum\limits_{k=1}^K 
% \int
% \left(
% \frac{P^{\rm DAT}(\lambda)}{P^{\rm DAT}(\lambda) + P^{\rm DAT}(\overline{\lambda})} \ell^{\rm DAT}(x_k \rightarrow x'_k, \lambda) \right. 
%\left.
% + \frac{P^{\rm DAT}(\overline{\lambda})}{P^{\rm DAT}(\lambda) + P^{\rm DAT}(\overline{\lambda})} \ell^{\rm DAT}(x'_k \rightarrow x_k,  \overline{\lambda})
% \right)
% \frac{P^{\rm DAT}(\lambda) + P^{\rm DAT}(\overline{\lambda})}{2}
% d\lambda
& = & \!\!\!\!\!\!
 \frac{1}{K}
 \sum\limits_{k=1}^K 
 \int
 \left(
 \frac{1}{2}P^{\rm DAT}(\lambda)
  \ell^{\rm DAT}(x_k \rightarrow x'_k, \lambda) \right. 
\left.
 + 
\frac{1}{2}P^{\rm DAT}(\overline{\lambda})
 \ell^{\rm DAT}(x'_k \rightarrow x_k,  \overline{\lambda})
 \right)
 d\lambda \\
& = & \!\!\!\!\!\!
 \frac{1}{2K}
 \left(
 \sum\limits_{k=1}^K 
 \int
 P^{\rm DAT}(\lambda)
  \ell^{\rm DAT}(x_k \rightarrow x'_k, \lambda) d\lambda
 + 
 \sum\limits_{k=1}^K 
 \int
 P^{\rm DAT}(\overline{\lambda})
 \ell^{\rm DAT}(x'_k \rightarrow x_k,  \overline{\lambda})
 d\lambda
 \right) \\
& \stackrel{(a)}{=} & \!\!\!\!\!\!
 \frac{1}{2K}
 \left(
 \sum\limits_{k=1}^K 
 \int
 P^{\rm DAT}(\lambda)
  \ell^{\rm DAT}(x_k \rightarrow x'_k, \lambda) d\lambda
 + 
 \sum\limits_{k=1}^K 
 \int
 P^{\rm DAT}(\lambda)
 \ell^{\rm DAT}(x'_k \rightarrow x_k,  \lambda)
 d\lambda
 \right) \\
& \stackrel{(b)}{=} & \!\!\!\!\!\!
 \frac{1}{2K}
 \left(
 \sum\limits_{k=1}^K 
 \int
 P^{\rm DAT}(\lambda)
  \ell^{\rm DAT}(x_k \rightarrow x'_k, \lambda) d\lambda
 + 
 \sum\limits_{k=1}^K 
 \int
 P^{\rm DAT}(\lambda)
 \ell^{\rm DAT}(x_k \rightarrow x'_k,  \lambda)
 d\lambda
 \right) \\
& = & \!\!\!\!\!\!
 \frac{1}{K}
 \sum\limits_{k=1}^K 
 \int
 P^{\rm DAT}(\lambda)
  \ell^{\rm DAT}(x_k \rightarrow x'_k, \lambda) d\lambda\\
 & = & \!\!\!\!\!\!
{\cal L}^{\rm DAT}
\left(
(x, x')_1^K
\right)
 \end{eqnarray*}
where (a) is due to a change of variable in the integration,  (b) is due to the symmetry of $(x, x')_1^K$.  \hfill $\Box$






\subsection*{ Proof of Theorem 4}
\begin{eqnarray*}
{\cal L}^{\rm uMix}_K\left((x, x')_1^K, \gamma \right) 
& = & 
\frac{1}{K} {\mathbb E}_{\lambda \sim P^{\rm Mix}} 
\sum\limits_{k=1}^K \left(
\gamma(\lambda) \ell^{\rm DAT}(x_k\rightarrow x'_k, \lambda)
+ \overline{\gamma(\lambda)} \ell^{\rm DAT}(x'_k\rightarrow x_k, \overline{\lambda})
\right) \\
& = & 
\frac{1}{K} 
\left(
{\mathbb E}_{\lambda \sim P^{\rm Mix}} 
\sum\limits_{k=1}^K 
\gamma(\lambda) \ell^{\rm DAT}(x_k\rightarrow x'_k, \lambda)
+ {\mathbb E}_{\lambda \sim P^{\rm Mix}} 
\sum\limits_{k=1}^K \overline{\gamma(\lambda)} \ell^{\rm DAT}(x'_k\rightarrow x_k, \overline{\lambda})
\right) \\
&\stackrel{(a)} {=} & 
\frac{1}{K} 
\left(
{\mathbb E}_{\lambda \sim P^{\rm Mix}} 
\sum\limits_{k=1}^K 
\gamma(\lambda) \ell^{\rm DAT}(x_k\rightarrow x'_k, \lambda)
+ {\mathbb E}_{\lambda \sim P^{\rm Mix}} 
\sum\limits_{k=1}^K \overline{\gamma(\lambda)} \ell^{\rm DAT}(x_k\rightarrow x'_k, \overline{\lambda})
\right) \\
&\stackrel{(b)} {=} & 
\frac{1}{K} 
\left(
{\mathbb E}_{\lambda \sim P^{\rm Mix}} 
\sum\limits_{k=1}^K 
\gamma(\lambda) \ell^{\rm DAT}(x_k\rightarrow x'_k, \lambda)
+ {\mathbb E}_{\overline{\lambda} \sim P^{\rm Mix}} 
\sum\limits_{k=1}^K \overline{\gamma(\overline{\lambda})} \ell^{\rm DAT}(x_k\rightarrow x'_k, \lambda)
\right) \\
%&= & 
%\frac{1}{K} 
%{\mathbb E}_{\lambda \sim P^{\rm Mix}} 
%\sum\limits_{k=1}^K \left(\gamma(\lambda) + \overline{\gamma(\overline{\lambda})} \right)
%\ell^{\rm DAT}(x_k\rightarrow x'_k, \lambda)\\
%&= & 
%\frac{1}{K} 
%{\mathbb E}_{\lambda \sim P^{\rm Mix}} 
%\sum\limits_{k=1}^K \left(\gamma(\lambda) -\gamma(\overline{\lambda})+1 \right)
%\ell^{\rm DAT}(x_k\rightarrow x'_k, \lambda)\\
%& = & 
%{\cal L}^{\rm wDAT}_K\left((x, x')_1^K , {\cal J}(\gamma) \right) 
& = &
\frac{1}{K} \sum\limits_{k=1}^K 
\int 
\left(
\gamma(\lambda) P^{\rm Mix}(\lambda)  \ell^{\rm DAT}(x_k\rightarrow x'_k, \lambda)
+ \overline{\gamma(\overline{\lambda})} P^{\rm Mix}(1-\lambda)  \ell^{\rm DAT}(x_k\rightarrow x'_k, \lambda)
\right)
d\lambda \\
& = &
\frac{1}{K} \sum\limits_{k=1}^K 
\int  \ell^{\rm DAT}(x_k\rightarrow x'_k, \lambda)
\underbrace{\left(
\gamma(\lambda) P^{\rm Mix}(\lambda)  
+ \overline{\gamma(\overline{\lambda})} P^{\rm Mix}(1-\lambda) 
\right)}_{{\mathbb D}_{\rm u}\left(P^{\rm Mix}, \gamma\right)}
d\lambda\\
& = & \frac{1}{K} \sum\limits_{k=1}^K {\mathbb E}_{\lambda \sim P^{\rm DAT}}  \ell^{\rm DAT}(x_k\rightarrow x'_k, \lambda)\\
& = & {\cal L}^{\rm DAT} \left((x, x')_1^K\right).
\end{eqnarray*}
where (a) is due to the symmetry of $(x, x'_1)^K$, and  (b) is by a change of variable in the second term (renaming $1-\lambda$ as $\lambda$).  \hfill $\Box$





